HeRo 2.0: A Low-Cost Robot for Swarm Robotics Research

The current state of electronic component miniaturization coupled with the increasing efficiency in hardware and software allow the development of smaller and compact robotic systems. The convenience of using these small, simple, yet capable robots has gathered the research community's attention towards practical applications of swarm robotics. This paper presents the design of a novel platform for swarm robotics applications that is low cost, easy to assemble using off-the-shelf components, and deeply integrated with the most used robotic framework available today: ROS (Robot Operating System). The robotic platform is entirely open, composed of a 3D printed body and open-source software. We describe its architecture, present its main features, and evaluate its functionalities executing experiments using a couple of robots. Results demonstrate that the proposed mobile robot is very effective given its small size and reduced cost, being suitable for swarm robotics research and education.

==> sections/3_design.tex <==
% HeRo Desing

This section presents all the stages for developing our robot ranging from mechanical and electrical design decisions to programming and simulations. Moreover, all decisions for our swarm robot considered the maximum use of commercially available components for ease of production and assembly and minimum possible price without sacrificing the processing power and sensing capabilities. \hec{Therefore, in the following, we present the best-suited system for HeRo after evaluating multiple microcontroller boards, wireless technologies, sensors, actuators, and model designs for additive manufacturing.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mechanical Design}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hec{One of the primary steps in developing a mobile robot is modeling its mechanics.} The process defines the kinematic model of the robot, its actuation mechanism, and also its structural design.

% \textcolor{red}{and measurement}

\subsubsection{Kinematic Model} 
After reviewing the literature, we observed that most robots proposed for swarm robotics are based on the differential-driven model. In a nutshell, a differential wheeled robot is a mobile robot whose movement is based on two separately driven wheels placed on either side of the robot body. The robot changes its direction by varying the relative speeds of its \hec{wheels, and therefore it does not require an additional steering motor. We also decided to implement such model since it is very suitable} for designing a small, low-cost robot that requires good maneuverability and speed using a simple actuation mechanism. 

\subsubsection{Actuators and Encoders} 
\label{sec:actuators}
A convenient and affordable way to actuate the wheels of a differential robot is the use of geared DC motors. Besides actuating the robot, these motors enable the use of encoders for computing odometry, which is important for localization and  closed-loop motion control.

Although it is intuitive to use geared DC motors with encoders, such components can significantly increase the cost of the robot. Thinking of a low-cost solution, we decided to use small continuous servo motors to actuate the robot's wheels. Such motor is similar to geared DC motors with an h-bridge component, allowing motor speed control. %However, the reduced cost and compact size of some commercially available servo motors make them an interesting solution for our robot. 

Besides having reasonable precision for speed control, continuous SG90 servo motors contain a built-in microchip that controls the motor speed and direction using only pulse-width modulation (PWM) signals. In addition, this motor has a significant torque of $1.8$~kgf/cm, which allows us to use a $5$~cm diameter wheel to reach a maximum linear speed of $25$~cm/s with $0.3$~kgf/cm of torque without losing traction. 

Instead of directly connecting the wheel to the motor shaft, we attach the wheel to the robot chassis and use a gear mechanism (1:1) to transmit torque from the motor to the wheel -- this further reduces backlash and wheel misalignment that impact the encoder readings.

Since such motor does not have a built-in encoder, we took advantage of larger wheels to design a mechanical transmission system (1:6) between the wheel and a mechanical rotary encoder. By considering the low cost, availability, and compact form, we selected Kailh rotary encoders. This encoder is widely used on mouse devices as a step counter for the scroll button, and the simplest models, like the ones we use, can count $48$~steps per cycle. However, performing the wheel-encoder transmission (1:288) increases the wheel position measurement to $1.25\degree$ degrees of resolution, which means that the robot detects a wheel step of $0.54$~mm when it is moving. Fig.~\ref{fig:herochassis} illustrates the motor-wheel and the wheel-encoder transmission system. The motor, rotary encoder, and wheel shaft are fixed to the robot chassis, and the other parts are moving.
%
\begin{figure}[!t]
  \centering
  \includegraphics[width=0.95\linewidth]{images/methodology/motor_transmission.pdf}
  \caption{Torque transmission mechanism from the motor to wheel and wheel to the rotary encoder. 
  %\todo{aumentar tamanho do texto dentro da figura}
  %\todo{daria para separar levemente as palavras das linhas? para ficar similares a como estão na Fig 3}
  }
  \label{fig:herochassis}
\end{figure}

\subsubsection{Structural Design}
\label{sec:structuraldesign}
After defining the actuation mechanisms, we proceed with designing the robot's chassis. To facilitate assembly and further extensions, we design the robot's chassis to be modular and 3D-printable so one can easily print it using a conventional 3D printer. Overall, the robot structure comprises four main parts: the motor and board chassis, cover, and the e-Hat module. 

The \textbf{motor chassis} supports both motors and the wheels shaft -- where the wheels are attached. As the robot has two actuated wheels, it has only two contact points on the ground. To better adjust the balance and alignment of the robot, we created two screwable castor wheels. These castor wheels are attached to the motor chassis and allow us to fine-tune the robot's balance. On top of the motor chassis, we attach the \textbf{board chassis} that holds the encoders, battery, and the main processing board.

Considering further extensions, we take advantage of a modular chassis to coin the concept of \textbf{e-Hat}. Such part is attached on top of the robot and works as a shield extending the robot's sensorial or acting capabilities. For instance, we developed an e-Hat with an IMU sensor. Other components, such as a camera, sonar, actuator, or even a UWB transceiver for indoor localization, can also be used.

Finally, we design a \textbf{cover} part to prevent dust accumulation inside the robot, protecting the main processing board and gears. In addition to protection, this part also enhances the robot's visual aesthetic. Fig~\ref{fig:heroexpanded} shows an expanded view of the robot's design. An interactive CAD visualization is available at A360 platform\footnote{Robot Design CAD: \url{https://a360.co/3lWHiv0}}.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.99\linewidth]{images/methodology/robot_desing.pdf}
  \caption{\hec{An expanded view of the robot's components and body parts.}}
  \label{fig:heroexpanded}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Electrical Design}
\label{sec:electricaldesign}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In parallel to the mechanical design stage, there is the electrical design of the robot. At this point, we define the electronic components built in the robot, such as processing unit, sensing, and power management.

\subsubsection{Microcontroller}
One of the major decisions concerning the robot's electrical design is the selection of an appropriate microcontroller. This component defines the robot's computational capacity and the number and variety of components we can use.

After considering many alternatives, we select the Espressif ESP8266 as the main processing unit. This microcontroller is \hec{remarkably} inexpensive given its excellent processing power (32-bit 160 MHz) with 4 MB of memory. Also, it has a built-in Wi-Fi microchip that provides a fast IEEE 802.11 connection with a full TCP/IP stack. So, the robots can communicate among them or with a remote computer using robust and scalable protocols. Moreover, it is efficient, easy to program, and widespread in Maker communities, \hec{allowing others to easily develop customized modules for the robot.}

% ATMEGA microcontrollers have been one of the top alternatives in the development of small, low-cost robots. Such microcontrollers are relatively inexpensive, efficient, easy to program, and widespread in Maker communities. However, this series of microcontrollers does not have much processing power, making it difficult to embed several components in the robot. So recent alternatives are the STM32 family and Raspberry Pi Pico boards that feature $32$-bits ARM Cortex processors. Both microcontrollers are extremely powerful, given their compact size, but they are also more expensive. 

% After considering many alternatives, we select the Espressif ESP8266 microcontroller. Besides being extremely inexpensive, it has excellent processing power ($32$-bit $160$~MHz) with a built-in Wi-Fi microchip that provides a fast IEEE $802.11$ connection with a full TCP/IP stack. So, the robots can communicate among them or with a remote computer using robust and scalable protocols.

\subsubsection{Sensing}
%Once the microcontroller is set, we define the sensors and components usually required in swarm robots. 
% like most other swarm platforms in the literature.

A important requirement for a small robot used in swarm experiments consists of measuring distances to neighboring robots and obstacles. In HeRo, we chose to use infrared sensors for this due to their size and cost. 
We arrange eight IR transmitters and receivers (TCRT5000) around the circumference of the robot with $45\degree$ increments. \hec{We selected such sensor because it is cost-effective and has a reasonable resolution and range.}

\hec{Although it is not common using this type of sensor for long distances (> 10 cm), we found a strategy to increase its range without a considerable decrease in accuracy by exploring the sensor saturation time.} In fact, the manufacturer defines the sensor's maximum range\footnote{TCRT5000: \url{www.vishay.com/docs/83760/tcrt5000.pdf}} to only $2$~cm. If the sensor is continuously powered, its sensitivity degrades due to some electrical saturation phenomenon. However, if we turn on the sensor for only a few microseconds, take the reading, and then turn it off, we can increase the detection range to up to $20$~cm. 

To control the power of the sensor, we use a MOSFET component. Due to the limited number of ADC pins on the microcontroller -- it only has one pin with 10-bits of resolution -- we have to include an 8-channel analog multiplexer enabling the microcontroller to read all the eight IR sensors. This setup allows us to precisely measure distances, avoiding environment light interference since we can measure it by using only the IR receivers. 

\hec{As mentioned earlier, the robot has two pairs of rotary encoders coupled to the wheels by a drive mechanism. An encoder is a sensor that generates digital signals in response to the motion, providing information about position, velocity, and direction. As the typical mouse wheel internally works as a precise encoder, we took advantage of this inexpensive component (less than USD $0.10$) and used it as a robotic sensor. 
%The mechanical encoder is highly comparable with other low-cost encoders in resolution (e.g., optical and magnetic encoders). 
It comprises a conductive disc and three contacts that generate two square waves in quadrature when the encoder shaft rotates, enabling counting $48$ pulses per shaft revolution and also identifying the turn direction. \rez{Thus, this mechanical encoder is highly comparable with other low-cost encoders in resolution (e.g., optical and magnetic encoders).}}

In addition to the encoders, the robot also houses two WS2812b RGBA LED indicators used for status monitoring or debugging. These addressable LEDs have an IC built right into the LED, allowing communication via a one-wire interface (it uses one digital pin to control multiple LEDs in series). We can also control the brightness, and the color of each LED individually, which allows us to produce unique and complex effects for status in a simple way.%\footnote{Video of LEDs indicators: \url{https://youtu.be/Ra7JX8Awkc0}}.

\subsubsection{E-Hat}
Besides the built-in features, the robot functionality can be extended using e-Hats. This robot module works as a shield, allowing users to create/customize specific modules for their applications. This module is coupled to a 4-pin bus on top of the robot configured to use I2C or UART protocols. In addition to communication, the bus also provides 5V (800 mA) to power the module. In this paper, we developed two e-Hats for demonstration and experimentation (see Figure~\ref{fig:ehats}). The first one consists of an e-Hat IMU composed of an MPU6050 sensor with gyroscope and accelerometer that can be fused into the velocity and position estimation to account for odometry errors, such as the slip produced by the wheels. The second one is an e-Hat display that can be used either as a user interface or as part of a location system based on camera and fiducial markers.

\begin{figure}[t]
    \begin{subfigure}{.49\textwidth}
      \centering
      \includegraphics[width=0.46\linewidth]{images/methodology/ehat_imu.pdf}
      \caption{\hec{IMU e-Hat.}}
      \label{fig:ehatimu}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
      \centering
      \includegraphics[width=0.92\linewidth]{images/methodology/e_hat_display.pdf}
      \caption{\hec{Display e-Hat.}}
      \label{fig:ehatdisplay}
    \end{subfigure}
\caption{\hec{Example of multiple e-Hat versions for the HeRo platform.}}
\label{fig:ehats}
\end{figure}

\subsubsection{Power Supply}

Since the robot's autonomy is an important factor considering the time and number of experiments, HeRo uses a 3.7 V 1800 mAh Li-Po battery. The battery voltage is regulated by a MT3608 DC-DC \hec{step-up module, managing the board power supply to $5$~V.} These components enable the robot to perform up to 3 hours of experiments, considering the continuous use of all components. The motors are directly powered by a step-up power module avoiding any voltage drop impacting the robot's speed. In addition to this module, we also use a TP4056 module to recharge the battery using a USB cable.

\subsubsection{Assembly}
\hec{Because most of the robot's parts are off-the-shelf components, we decided to simplify the mounting and wrap them right on a PCB board. To increase reproducibility, we carefully design this PCB board so that even novice users can assemble it. As an alternative, the user can also assemble it in several specific PCB manufacturers, which nowadays attend at a highly affordable cost. Fig.~\ref{fig:herodesign} shows the proposed front and back views PCB board's design.}

%The figure shows the PCB board's design and, on the side, a PCB board purchased from one of these manufactures and assembled in our laboratory.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.9\linewidth]{images/methodology/board_sketch.pdf}
  \caption{\hec{Overview of HeRo's PCB board.}}
  \label{fig:herodesign}
\end{figure*}

\subsubsection{Part Costs}
Table~\ref{table:parts_cost} gives a summary of the cost of the components used in HeRo. \hec{All part prices assume retail buying from standard part distributors on the Internet.} We expect this cost would be greatly reduced if parts are acquired in bulk directly from manufacturers.

\begin{table}[!t]
\centering
	\caption{Parts cost per robot \hec{unit}.}
	\label{table:parts_cost}
	\scalebox{0.42}{
	\resizebox{\textwidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Parts} & \textbf{Quantity} & \textbf{Cost (USD)} \\
\midrule
Servo Motors SG-90 & 2 & 2.06 \\
Mouse Encoder 48 PPR & 2 & 0.10 \\
ESP8266 Nodemcu & 1 & 2.50 \\
Rubber O Ring 38mm & 2 & 0.10 \\
IR TCRT5000 & 8 & 0.68 \\
LED RGB WS2812b & 2 & 0.51 \\
IMU MPU6050 & 1 & 0.85 \\
LI-PO Battery 3.7 V 1800 mAh & 1 & 5.85 \\
PCB board and Components & 1 & 4.30 \\
3D Printer Parts (ABS) and Fastening & 1 & 1.50 \\
\midrule
\textbf{Total} &  & 18.72 USD\\
\bottomrule
\end{tabular}}}
\end{table}

Finally, after carrying out the robot assemblies, we arrived at the result shown in the Fig.~\ref{fig:heroreal}.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.90\linewidth]{images/methodology/hero_view.png}
  \caption{Top, bottom, front, and left views of \hec{the HeRo swarm platform.}}
  \label{fig:heroreal}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Software Architecture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% One of the most typical dilemmas in robot swarm systems is the convenience of promptly programming multiple robots. This work proposes a diversified architecture that enables the user to implement swarm applications promptly, efficiently, and elegantly. 

% The proposed software architecture allows the robots to be remotely programmed and executed remotely on a computer or locally on the robot. The first programming strategy follows the development strategy using middleware ROS, one of the most popular platforms for robotics. To make the robot ROS-Compatible we implement a firmware that interfaces the ROS by topics and services using ROSSerial protocol. Such an approach allows the users to create their applications in several programming languages ​​and control multiple robots remotely using TCP/IP networking. The second strategy follows the OTA (Over-The-Air) technology that allows the user to burn the robot's firmware via a Wi-Fi interface remotely.

% In the following, we detail the implementation of each module of our firmware as well as the communication process, programming framework, simulation and visualization. Figure \ref{fig:software_architecture} shows an overview of how these modules interact to each other as well as the user's applications. 

A typical robot swarm dilemma is how to program multiple robots \hec{quickly}, easily, and efficiently. A practice that has become very common in the experimentation stage is to use a master-slave architecture in which robots (slaves) remotely communicate with a computer (master) running the user application. This strategy is highly efficient as it does not require the user to burn the firmware every time he needs to change his application. Despite being convenient, remotely executing the application on a computer does not always capture effects that impact the application at the deployment level, e.g., local communication issues, low processing capacity, and other errors. Thus, strategies that use FOTA (Firmware Over-The-Air) technology enable users to remotely load their applications on the robot and run it directly on it.

In this work, we propose a flexible architecture to use any of the programming practices mentioned above. Our architecture is composed of a firmware compatible with ROS (Robot Operating System) and FOTA. In the following, we detail the software architecture.

\subsubsection{Firmware}

The firmware is one of the fundamental parts of the robot since it provides low-level control for the motors and access to the sensor's data. For HeRo, we chose to implement the firmware using the Arduino IDE. Such platform is easy to use and widespread in makers' communities, making the firmware easier to follow and modify. It also provides many libraries enabling us to control the microcontroller ports and handle actuators, sensors, and TCP sockets. 

The firmware is built on top of the rosserial framework allowing the robots to be compatible with the ROS middleware. Rosserial comprises different tools, including a protocol for wrapping standard ROS serialized messages and multiplexing multiple topics and services over network sockets. Such framework abstracts several communication concepts, allowing a compact and efficient implementation. In practice, the user only needs to configure a few communication parameters so that the robots can connect using TCP/IP networking with a remote computer running ROS. To facilitate this configuration process, we implemented a remote configuration mode for the robot using a web interface (Fig.~\ref{fig:heroconfig}). 
%To reach such a interface the users should connect to an access point created by the robot. 
\hec{To open this interface, the users should connect to an access point created by the robot. Once the robot is properly configured, it can connect to the user's network allowing the user to interact with the robot's features through topics and services. This entire process can be done in less than a minute.}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.6\linewidth]{images/methodology/webconfig.pdf}
  \caption{Configuring the robots to connect to a server running ROS only requires  the connection with an access point raised by the robot. Then, using a web configuration platform, robot connection parameters can be easily modified.}
  \label{fig:heroconfig}
\end{figure*}

In addition to providing a master-slave communication architecture, the firmware is also composed of some basic modules that compute the robot's cinematic control, odometry, and sensor data. Next, we describe all \hec{these modules present in the firmware.}

\paragraph{\textbf{Sensors}}
In its basic form (without the e-Hat), the robot has eight infrared transceivers and two quadrature mechanical rotary encoders as sensors. The eight infrared sensors are mounted around the robot to provide a complete field-of-view of the environment.  These are connected to a 10-bits ADC port on the microcontroller through an 8-channel analog multiplexer allowing the estimation of the distance to an obstacle as well as the ambient light once we can control the infrared emitter. Obstacle detection and distance estimation use fundamental principles of electromagnetic radiation and its reflection. Mathematically, the reflected signal intensity measured with a sensor is modeled by~\cite{benet2002using}:

\begin{equation}
    \label{eq:infrared}
    s(x, \theta) = \frac{\alpha}{x^2} cos(\theta) + \beta,
\end{equation}

where $s(x, \theta)$ is the output value of the sensor, $x$ is the distance to the object, and $\theta$ is the angle of incidence with the surface; the model variable $\alpha$ includes several parameters such as the reflectivity coefficient, output power of the emitted IR light and the sensitivity of the sensor and it is estimated empirically; $\beta$ is the offset value of the amplifier and ambient light effect and it is measured regularly after performing the Equation~\ref{eq:infrared}. 

As mentioned, HeRo has two quadrature encoders attached to each wheel. A quadrature encoder, also known as an incremental rotary encoder, is commonly used to measure the speed and direction of a rotating shaft. The encoders' channels are connected to the microcontroller's interrupt pins. \hec{Each pulse calls an interrupt routine in the microcontroller, increasing an independent counter variable} to estimate how far each wheel has turned. To estimate the velocity of the wheel, we measure the frequency of the pulses. The output of the encoders is used as an input to a controller for closed-loop motion control and for localization.

\paragraph{\textbf{Odometry}}
Odometry is the most used method for determining the momentary position of a mobile robot. In most practical applications, odometry provides easily accessible real-time positioning information in-between periodic absolute position measurements. Several different types of sensors are commonly used for odometry. \hec{This work addresses odometry by placing encoders on each wheel} and counting how far each wheel has turned. Using these two measurements we can estimate how far the robot has moved forward and its heading. The distance traveled by the robot is computed by the average of how much each wheel has turned and is presented in Equation~\ref{eq:wheel_travel}. On the other hand, the heading of the robot is estimated (assuming insignificant wheel slip) from the difference of these displacements over the distance between the wheels and is presented in Equation~\ref{eq:wheel_turn}.
%\hec{Both equations are presented below:}
\begin{equation}
\label{eq:wheel_travel}
\Delta L =  \frac{\Delta\theta_r r_r + \Delta\theta_l r_l}{2},
\end{equation}
\begin{equation}
\label{eq:wheel_turn}
\Delta\theta =  \frac{\Delta\theta_r r_r - \Delta\theta_l r_l}{l},
\end{equation}
where $\Delta\theta_r$ and $\Delta\theta_l$ represents how much each encoder has turned in the time interval; $r_r$ and $r_l$ are the right and left wheel radius; and $l$ represents the distance between the wheels of the robot.

\hec{Once we have computed how far the robot has traveled and turned, we can integrate this information to estimate its current pose.} Considering the pose of the robot at time $t$ in a plane is given by the state vector $X(x(t), y(t), \theta(t))$, the next pose of the robot at time $t + 1$ is given by 
%
\begin{equation}
\scalemath{0.76}{
X(t+1) = 
\begin{bmatrix}
x(t+1) \\ 
y(t+1) \\ 
\theta(t+1)
\end{bmatrix}
=
\begin{bmatrix}
x(t) + \frac{\Delta L}{\Delta \theta} (sin(\theta(t) + \Delta\theta) - sin(\Delta \theta)\\ 
y(t) + \frac{\Delta L}{\Delta \theta} (cos(\theta(t) + \Delta\theta) - cos(\Delta \theta)\\ 
\theta(t) + \Delta\theta
\end{bmatrix}.
}
\end{equation}
%
However, this model does not explain the position increment when the robot performs straight forward movements. In this case,  we have $\Delta\theta = 0$ and this makes $\frac{\Delta L}{\Delta \theta}$ undefined. In order to approach this special case, we test this condition and if it occurs the following model is computed for the odometry
%
\begin{equation}
X(t+1) = \begin{bmatrix}
x(t+1) \\ 
y(t+1) \\ 
\theta(t+1)
\end{bmatrix}
=
\begin{bmatrix}
x(t) + \Delta L  cos(\theta(t))\\ 
y(t) + \Delta L  sin(\theta(t))\\ 
\theta(t)
\end{bmatrix}.
\end{equation}

\paragraph{\textbf{Motion Control}}

% Previously, we define the robot as a two-wheel differential-drive mobile robot composed of two servo motors each with a quadrature encoder. A differential wheeled robot is a mobile robot whose movement is based on two separately driven wheels placed on either side of the robot body. It can thus change its direction by varying the relative rate of rotation of its wheels and hence does not require an additional steering motor. To control the velocity of the mobile robot, the mathematical model of the robot kinematics and a suitable controller should be implemented. Mathematical modeling of the robot kinematics is one of the major parts of the control system in robot design. In short, this model takes the velocities of the actuators and transform them into the generalized coordinate vector. To control our robot, the high-level velocities with respect to the tangential velocity on each wheel is computed by the inverse kinematic model, 

%To control our robot, the high-level velocities with respect to the mobile robot are related to the tangential velocity on each wheel by the inverse kinematic model, 

\hec{Previously, we defined the robot as a two-wheel differential-drive mobile robot composed of two servo motors, each with a quadrature encoder. The robot can change its direction by varying the relative rotation rate of its wheels and hence does not require an additional steering motor. The inverse kinematic model computes the tangential velocity on each wheel given a set of high-level velocities using the following equations,}
%
\begin{equation}
\begin{bmatrix}
v_{l}(t) ~ v_{r}(t)
\end{bmatrix}^T 
=  \begin{bmatrix}
\frac{2v(t) - l\omega(t)}{2} ~ \frac{2v(t) + l\omega(t)}{2}
\end{bmatrix}^T,
\end{equation}
where $v_{l}(t)$ and $v_{r}(t)$ are the tangential velocities of the left and right wheels; $v(t)$ and $\omega(t)$ are the high-level linear and angular velocities of the mobile robot; and $l$ is the distance between the left and right wheels.

Once computed the tangential velocities on each wheel, we need to control the motors \hec{so} that they maintain these velocities. The proportional-integral-derivative controller (PID controller) is the most common control algorithm used for this application. It \hec{can} correct the present error through proportional action, eliminate steady-state offsets through integral action, and better estimate the future trends through a derivative action. The mathematical model of a PID is defined by
%
\begin{equation}
u(t) = K_{p}e(t)+K_{i} \int _{0}^{t}e(t')\,dt' + K_{d}{\frac {de(t)}{dt}},
\end{equation}
where $u(t)$ is the control signal to each motor; $e(t)$ is the error regarding the tangential velocity of each wheel; and $K_{p}$, $K_{i}$ and $K_{d}$, all non-negative, denote the coefficients for the proportional, integral, and derivative terms, respectively. \hec{To estimate the error, we subtract the tangential velocity obtained by the inverse kinematic model from the tangential velocity estimated by the encoders. A Kalman} filter is used to reduce the reading noise estimated by the encoder. Figure \ref{fig:overview_motion_control} shows an overview of this controller.

%% Atualizar figura.... filtro de kalman
\begin{figure}[]
      \centering
      \includegraphics[width=0.95\linewidth]{images/methodology/motion_control.pdf}
      \caption{Diagram of the controller used for closed-loop velocity control.}
      \label{fig:overview_motion_control}
\end{figure}

% PID tuning comprises of setting the best value of $K_p$, $K_i$ and $K_d$ of the PID so that the system performance can be increased. The proportional terms have the effect of reducing the rise time but never eliminate the steady-state error. The integral terms have the effect of eliminating this steady-state error, but can make the transient response worse. The derivative term has the impact of increasing the stability of the system, reducing the overshoot, and improving the transient response. After properly tuning the PID terms our controller is able to perform the velocity control on the robot's wheels. Figure \ref{fig:overview_motion_control} shows an overview of this controller.



\subsection{Communication Architecture}
%\todo{falar de west2018ros, trabalho que mostra que utilizar protocolo rosserial e escalavel para swarm...} \cite{west2018ros}

% fundir isso com o que foi falado antes...
In order to provide communication between a workstation and the robots, we implement HeRo as a \hec{ROS-compatible robot by connecting them using TCP/IP.}

The Robot Operating System~\cite{quigley2009ros} is an open-source, meta-operating system for robotic applications. It provides similar services expected from a typical operating system, including hardware abstraction, low-level device control, implementation of commonly-used functionality, message-passing between processes, and package management. It also provides tools and libraries for obtaining, building, writing, and running code across multiple platforms.

The communication is conducted by a publish/sub\-scribe model, where topics made up of predefined message structures can be communicated between multiple nodes (processes) in the network. These topics, for example, odometry, can be accessed by any node in the network, allowing for easy scalability of publishers and subscribers. In this way, robots can readily communicate with other robots in the network in a well-defined way. 

%However, most instances of swarm robots, including HeRo, are very limited to process native ROS instance. In %nearly all cases, researchers are unable to provide the functionalities of the swarm robot in ROS, since they are not able to locally run the ROS core -- a collection of process and programs that are pre-requisites of a ROS-based system.

\hec{However, most swarm robots, including HeRo, are unable to process a full-fledged native ROS instance given the restricted CPU resources. To integrate these functionalities to less powerful microcontrollers without a complete instance of ROS, we implemented the communication module over the rosserial protocol. Rosserial\footnote{http://wiki.ros.org/rosserial} is a protocol for wrapping standard ROS serialized messages and multiplexing multiple topics and services over a network socket.}

In short, the rosserial nodes convert data from normal structured XMLRPC protocol handled by TCP natively in ROS to serialize data out to the microcontroller. This node also deserializes data from the microcontroller back into the correct message structures to be sent around the conventional ROS network. Figure \ref{fig:communication_architecture} shows an overview of this process. %The rosserial protocol has been validated as a reliable and scalable communication method for swarm systems~\cite{west2018ros}.

\begin{figure}[!t]
      \centering
      \includegraphics[width=0.96\linewidth]{images/methodology/communication_architecture.pdf}
      \caption{An overview of the communication process. The robot's microcontroller acts as a bridge to the sensors and actuators and then rosserial acts as another bridge from the microcontroller to ROS.}
      \label{fig:communication_architecture}
\end{figure}

\hec{In theory, the network's bandwidth limits the number of connected robots: as more robots are added, more connections are made, taking up capacity. However, we did not observe any overhead communicating with multiple robots, even using a consumer-grade wireless network router. A typical network addresses 254 devices, but network techniques (e.g., subnets) allow increasing this limit as much as we need. A complete study showing the reliability and scalability of using this protocol for swarm robots is present in~\cite{west2018ros}.}

\subsection{Simulation and Visualization}
% melhorar essa parte, atualizar essa parte

%\hec{Although programming directly on a real robot can provide genuine feedback and is more impressive than simulations, simulators play an essential role in robotics research as tools for quick and efficient testing of new concepts, strategies, and algorithms. For this reason, we also provide a simulated model of HeRo.}

The execution of simulations plays an essential role in robotics research as tools for quick and efficient testing of new concepts, strategies, and algorithms. Moreover, good visualization tools are very important during the experiments to better track and observe the robot execution. In this sense, we also developed a simulation model of HeRo that can be used together with Gazebo and RViz. 


\subsubsection{Gazebo Simulator}
In order to make simulations with our robots in ROS, we decide to use Gazebo since it is fully integrated with ROS. Gazebo~\cite{koenig2004design} is a multi-robot simulator for complex indoor and outdoor environments. It is suitable for simulating a population of robots, sensors, and objects in a three-dimensional world. \hec{ROS and Gazebo use the 3D model of a robot or its parts, whether to simulate or visualize them, through the XML files, called Unified Robot Description Format (URDF). This file describes all the structures of the robot, such as its parts, joints, dimensions, and texture, among others.}

After describing the robot using the URDF file, creating a simulated model using  the built-in plugins provided by the Gazebo is straightforward. However, this approach is inefficient when simulating multiple robots and requires a high computational cost. To reduce consumption and increase the number of simulated robots, we designed a compact plugin that implements all the robot's functionalities. In this way, we optimized the maximum processing performed by each simulated robot without overloading Gazebo's physics engine. Fig.~\ref{fig:hero_gazebo} shows multiples instances of HeRo being simulated in the Gazebo simulator.

\begin{figure}[]
      \centering
      \includegraphics[width=0.95\linewidth]{images/methodology/gazebo.jpg}
      \caption{Multiple instances of HeRo being simulated in the Gazebo simulator.}
      \label{fig:hero_gazebo}
\end{figure}

\subsubsection{Visualization Tool}

\hec{Once we have a 3D model and the robot's descriptions we generate the configuration file necessary for RViz. We associate the robot's parts, such as chassis and wheels, named links, through joints. Once this description file is generated, we can visualize the robot in ROS using the RViz visualization tool. This tool provides 3D visualization of the robot by loading the URDF file and associating its joints to the transform tree, which animates the model. In addition to displaying the robot model, RVIz can project sensors data such as} odometry, laser, and IMU using plugins. Note that RViz is not a simulator but only a visualization tool. In this way, the robot visualized in this tool can be real or simulated depending only on who publishes the information. Fig.~\ref{fig:hero_rviz} shows an example of viewing the robot in Rviz. Colored objects in the rectangular shape can move closer or further away from the robot, indicating the readings from the distance sensors. The grey shape on the floor represents part of a map built by the robot.

\begin{figure}[]
      \centering
      \includegraphics[width=0.95\linewidth]{images/methodology/rviz.png}
      \caption{RViz showing a single HeRo with the transform tree (colored axis). RViz is a 3D visualization tool for ROS allowing control and observe the current state of the robot.}
      \label{fig:hero_rviz}
\end{figure}

\subsection{Programming}
The communication architecture defined for our robot allows it to be programmed in two different ways: using the ROS framework or the OTA firmware technology.

In the first mode, we can program and run applications on a server, which communicates and controls each robot in a decentralized way. In other words, each algorithm is executed in a process on the server, and this process has access via Wi-Fi with its respective robot. This mode is very convenient and scalable in the early stages of testing with multiple robots. Furthermore, using the ROS framework for implementation, we have a series of tools and may use different programming languages.

On the other hand, processing algorithms remotely is not always ideal for robot swarm applications. In this case, the algorithm must run directly on the robot, maintaining the convenience of robot programming. The robot also allows remote burning of the firmware using Wi-Fi. However, it is limited in terms of the availability of high-level tools and programming languages. In this mode, one can use the Arduino IDE for programming the robots.

% firmware ros compatible
% controls & filter
% architecture
% communication
% web setup interface
% scalability
% rviz
% Gazebo

% \todo{\\
% - Colocar examples programacao ros e FOTA}
% ros examples
% arduino ide fota


==> sections/temp.tex <==
%%%%%%%%%%%%%%%%%%
% Hero evolution
%%%%%%%%%%%%%%%%%%
% With such constraints in mind, we investigate the most common and affordable components suitable to reach the best design. We explored different microcontroller boards (e.g., Arduino Uno, Nano, and Mini Pro and also ESPressif ESP8266), wireless technologies (Wi-Fi, Bluetooth, and Radio Frequency), actuators (DC Motors, Stepper Motors, and Servo Motors), and model designs for 3D printing. 

% Figure \ref{fig:all_heros} shows all versions of HeRo and Table \ref{table:hero_versions} shows a comparison between them. In the following, we present the design process of the current version on HeRo.

% MELHORAR FOTOS %
% \begin{figure}[t]
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       \includegraphics[width=0.74\linewidth]{images/herov01.png}
%       \caption{Version 0.1 (2016);%\footnote{HeRo v0.1: \url{https://youtu.be/jat3IoTiILY}} 
%       }
%       \label{fig:herov01}
%     \end{subfigure}
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       \includegraphics[width=0.72\linewidth]{images/herov1.png}
%       \caption{Version 1.0 (2017);%\footnote{HeRo v1.0: \url{https://youtu.be/TsN\_MTOrzfk}}
%       }
%       \label{fig:herov1}
%     \end{subfigure}
%     \begin{subfigure}{.50\textwidth}
%       \centering
%       \includegraphics[width=0.28\linewidth]{images/hero.pdf}
%       \caption{Version 2.0 (2020);}
%       \label{fig:herov2}
%     \end{subfigure}
% \caption{ HeRo's design evolution.}
% \label{fig:all_heros}
% \end{figure}

% \begin{table*}[t]
% \centering
% \caption{Comparison among all version of our robot.}
% \label{table:hero_versions}
% \resizebox{\textwidth}{!}{\begin{tabular}{llll}
% \toprule
%  & HeRo v0.1 & HeRo v1.0 & HeRo v2.0\footnote{HeRo v2.0: \url{HeRo v2.0}} \\
%   \midrule
% Board & Arduino Nano & ESPressif ESP8266 - ESP12 & ESPressif ESP8266 - ESP12 \\
% MCU & Atmel Atmega328 8-bit @ 16 MHz & Tensilica LX106 32-bit @ 80/160 MHz & Tensilica LX106 32-bit @ 80/160 MHz \\
% Communication & RF nrf24l01 2.4 Ghz & Wi-Fi 802.11bgn & Wi-Fi 802.11bgn \\
% Actuation & Servo Motors & Servo Motors & Servo Motors \\
% Footprint & 10 cm & 8 cm & 6.7 cm \\
% Sensors & None & 3 x infrared sensors & 8 x infrared sensors, encoders and IMU \\
% Battery & 3.7 V 1000 mAh Li-Po & 3.7 V 1000 mAh Li-Po & 3.7 V 1800 mAh Li-Po \\
% Cost* & \$ 9.00 & \$ 14.00 & \$ 18.00 \\
% \bottomrule
% * current cost of the parts &
% \end{tabular}}
% \end{table*}
